Non-orientable slice surfaces and inscribed rectangles

We discuss differences between genera of smooth and locally-flat non-orientable surfaces in the 4-ball with boundary a given torus knot or 2-bridge knot. In particular, we establish that a result by Batson on the smooth non-orientable 4-genus of torus knots does not hold in the locally-flat category. We further show that certain families of torus knots are not the boundary of an embedded M\"obius band in the 4-ball and other 4-manifolds. Our investigation of non-orientable surfaces with boundary a given torus knot is motivated by our approach to unify the proof of the existence of inscribed squares and of inscribed rectangles with aspect ratio $\sqrt3$ in Jordan curves with a regularity condition. This generalizes a result by Hugelmeyer for smooth Jordan curves.

==> parts/upperboundsongamma4_old.tex <==
% !TEX root = ../squarepeg.tex

\newcommand{\gtop}{\gamma_4^{\rm top}}
\newcommand{\gsmooth}{\gamma_4}
\newcommand{\gstop}{\gamma_4^{\rm stop}}
\newcommand{\gssmooth}{\gamma_4^{\rm s}}

\section{Non-orientable $4$--genus for torus knots in $S^3$}\label{s:balls}

In this section we discuss non-orientable $4$--genus for torus knots in $S^3$. In Subsection~\ref{subsec:ProofThm1.3}, we show that for torus knots the notion of non-orientable $4$--genus depends on the choice of category by establishing the existence of locally-flat surfaces in $B^4$ with boundary certain torus knots. In contrast, in Subsection~\ref{subsec:mob}, we discuss obstructions (in both categories) for the existence of Möbius bands in $B^4$ with boundary a given knot.

We begin by setting up the notation and collecting some facts we will need throughout the section.

We denote with $\langle q \rangle$ the bilinear form $x\otimes y \mapsto xqy$; we use the same notation for bilinear forms that take values in $\Z$ (like the intersection form of a $4$--manifold with $b_2 = 1$) and for those that take values in $\Q/\Z$ (like the linking form $\lambda_Y$ of a rational homology $3$--sphere $Y$ with cyclic $H_1$).
We denote with $\big(\frac pq\big)$ the Jacobi symbol.
We say that a linking form $\lambda_Y$ \emph{represents $s$ as a square} if there exists a torsion element $x \in H_1(Y)$ such that $\lambda_Y(x,x) = s$.

The following statement is a special case of a result of Murakami and Yasuhara~\cite{MurakamiYasuhara}.

\begin{prop}[{\cite[Corollary~2.7]{MurakamiYasuhara}}]\label{p:MY}
Let $K\subset S^3$ be a knot that bounds a locally-flat M\"obius band in $B^4$ and such that $\det K$ is square-free. Then the linking form on $\Sigma(K)$ represents $1/|{\det K}|$ or $-1/|{\det K}|\in \Q/\Z$ as a square.
\end{prop}

Recall that, if $p$ is even and $q$ is odd and coprime with $p$, then $|{\det T_{p,q}}|= |q|$.
Recall also that the double cover of $S^3$ branched over $T_{p,q}$ is the manifold $\Sigma(2,p,q)$, i.e. the link of the singularity of $\{x^2+y^p+z^q = 0\} \subset \C^3$ at the origin.

\begin{lemma}\label{l:surgerypresSigmatorus}
The $3$--manifold $\Sigma(2,2n,2n\pm1)$ is the boundary of a $4$--manifold $W$ with $H_1(W) = H_3(W) = 0$ and whose intersection form is represented by the matrix $\big({\tiny\begin{array}{cc}\mp n - 1& n\\n& \mp n - 1\end{array}}\big)$.
\end{lemma}

\begin{proof} 
The $4$--manifold $W$ is given as the trace of the surgery in Figure~\ref{f:Sigma245}. We first unknot $T_{2n,2n\pm 1}$ with an axial surgery (left); the corresponding link is symmetric, so we swap its components (center); finally, we branch double cover over the axis (right).
The framings are easily computed (see, for example,~\cite[Section 10.C]{Rolfsen}) to be $\mp n - 1$ for each of the two $2$--handles, and their linking number is $\pm n$ (the signs are coherent with the sign determining the knot).
Up to changing the orientation of one of the two components, we can always change the signs off the diagonal, so the intersection form is presented by the matrix $\big({\tiny\begin{array}{cc}\mp n - 1& n\\n& \mp n - 1\end{array}}\big)$.
\end{proof}

\begin{lemma}\label{l:presentingassquares}
Let $p$ be a prime and $\lambda$ be a linking form on $\Z/p\Z$ that represents $-\frac1p$ as a square.
\begin{enumerate}
\item\label{linking2mod4} If $p\equiv 5 \pmod 8$, then $\lambda$ represents neither $\frac2p $ nor $-\frac2p$ as squares.
\item\label{linking3mod4} If $p \equiv 7 \pmod 8$, then $\lambda$ represents $-\frac2p$ as a square, but not $\frac2p$.
\end{enumerate}
\end{lemma}

\begin{proof}
Since $\lambda$ represents $-\frac1p$, $\lambda$ is isomorphic to $\langle -\frac1p \rangle$; that is, $\lambda(x,x) = -\frac{x^2}p$ for every $x \in \Z/p\Z$, and $\frac{2}{p}$ (respectively, $-\frac{2}p$) is represented as a square if and only if $\jacobi{-2}{p} = 1$ (resp. $\jacobi{2}{p} = 1$).

It is well-known that $\jacobi{-1}{p} = 1$ if and only if $p\equiv 1 \pmod 4$, and that $\jacobi{2}{p} = 1$ if and only if $p\equiv \pm 1 \pmod 8$ (see, for instance,~\cite[Theorems~82 and~95]{HardyWright}). Using multiplicativity of Legendre symbols, we quickly derive both statements.
\end{proof}

\subsection{Proof of Theorem~\ref{thm:gammafortorusknots}}\label{subsec:ProofThm1.3}
The following proposition is a strengthening of Theorem~\ref{thm:gammafortorusknots}.

\begin{prop}\label{prop:gammatop<gammasmooth}
For integers $n\geq5$, we have $\gtop(T_{2n-1,2n}) \le n-2 < n-1 = \gsmooth(T_{2n-1,2n})$.

In fact, there exists a non-orientable connected locally-flat surface $\Sigma\subset B^4$ with $b_1(\Sigma)=n-2$ such that $\partial \Sigma=T_{2n-1,2n}$ and $\pi_1(B^4\setminus \Sigma)\cong \Z/2\Z$.

If $2n-1$ is a prime congruent to $5$ modulo $8$, then $\gtop(T_{2n-1,2n}) \ge 2$.
\end{prop}

\begin{remark}
Recently, Lobb observed in~\cite{Lobb19} that $\gsmooth$ is smaller on torus knots than previously conjectured by Batson in~\cite{Batson}.
However, one may ask whether the conjecture holds when restricting to surfaces with complements that have cyclic fundamental group.
(Note that, by the Mayer--Vietoris sequence, the first homology of the complement of such a surface is always $\Z/2\Z$.)
The second assertion of the above proposition, implies that even in this more restrictive setup, the topologically locally-flat quantity is strictly smaller than the corresponding smooth one.
\end{remark}

\begin{proof}[Proof of Proposition~\ref{prop:gammatop<gammasmooth}]
The equality $n-1 = \gsmooth(T_{2n-1,2n})$ is due to Batson.
For the upper bound on the topological cross cap number, we find a non-orientable spanning surface $S \subset S^3$ for $T_{2n-1,2n}$ with $b_1(S) = n$ with the following property: there is a separating simple closed curve $\gamma \subset S \subset S^3$ with trivial Alexander polynomial, such that one of the two connected components of $S\setminus\gamma$ is a once-punctured torus.

We modify $S$ by replacing the once-punctured torus in $S^3$ with the locally-flat disc in $B^4$ with boundary $\gamma$. By doing so, we find a locally-flat non-oriented surface $\Sigma \subset B^4$ with $b_1(\Sigma) =n-2$ that fills $T_{2n-1,2n}$.
The existence of such a disc is guaranteed by a consequence Freedman's celebrated disk theorem: knots with Alexander polynomial one are topologically slice.
In fact, a knot $K$ has Alexander polynomial $1$ if and only if, there exists a locally-flat disc $D\subset B^4$ with boundary $K$ such that $\pi_1(B^4\setminus D)\cong\Z$; see~\cite[Theorem~1.13]{Freedman_82_TheTopOfFour-dimensionalManifolds}. A Seifert--van Kampen calculation allows to check that the complement of $\Sigma$ (pushed into $B^4$ to be properly embedded) has cyclic fundamental group; this follows from the fact that $\pi_1(B^4\setminus D)\cong\Z$. In the rest of the proof we implement this in detail.

We first describe a (non-orientable) spanning surface $S$ for $T_{2nk-1,2n}$ for $k\geq0$. While we are interested in the case $k=1$, it is instructive to see that all of these are built from the case $k=0$. For this, we view $T_{2nk-1,2n}$ as the closure of the $2n$--stranded braid $(\sigma_1\sigma_2\cdots \sigma_{2n-1})^{2kn-1}$.
For $k=0$, we take $S$ to be the checkerboard surface for the standard diagram of the braid closure of $(\sigma_1\sigma_2\cdots \sigma_{2n-1})^{-1}$ that misses the braid axis. For $k\geq 1$, we take $S$ to be the surface obtained from the one for $k=0$ by $k$--surgery along the braid axis; i.e.~by adding $k$ positive full twists as depicted in Figure~\ref{fig:S}. Note that $b_1(S)=n$.
\begin{figure}[ht]
\centering
\subcaptionbox{\label{fig:Fzero} The spanning surface $S$ (blue).}
{\def\svgscale{0.7}
\centering
\input{figures/twist.pdf_tex}}
\subcaptionbox{\label{fig:alphasinFzero} The curves $\alpha_i$: $\alpha_{i+1}$ is a copy of $\alpha_i$ shifted down by two strands. }
{\def\svgscale{1.5}
\centering
\input{figures/curvesonS.pdf_tex}}
\caption{\label{fig:S}The surface $S$ and the curves $\alpha_i$ on $S$. The curves $\alpha_i$ and $\alpha_{i+1}$ intersect in one point. The box represents $k$ positive full twists on $2p$ strands.}
\end{figure}


Next, we define an orientable, incompressible subsurface $F$ of $S$ with $b_1(F)=n-1$.
Let $\alpha_1$, $\alpha_2$, $\dots$, $\alpha_{n-1}$ be the simple closed curves depicted in Figure~\ref{fig:S}, and take $F$ to be a neighborhood of their union; in particular, the homology classes of the $\alpha_i$ constitute a basis for $H_1(F;\Z)$.
We focus on $F$ and try to find a separating curve in $F$ with Alexander polynomial one that cuts out a once-punctured torus. The boundary of a once-punctured torus $T$ is a knot with Alexander polynomial $1$ if and only if one (and thus all) matrix $A$ representing the Seifert form on $T$ satisfies
\begin{equation}\label{eq:Alex1}
\det(t^{1/2}A-t^{-1/2}A^T)=1.
\end{equation}
Therefore, finding such a once punctured torus amounts to finding a pair of once-intersecting curves $\beta_1$ and $\beta_2$ in $F$ such that, if $A$ is the matrix representing the restriction of the Seifert form on $F$ to ${\rm span}\{[\beta_1],[\beta_2]\}\subset H_1(F,\Z)$, then $A$ satisfies~\eqref{eq:Alex1}.
In fact, it suffices to find a rank-two subgroup $H$ of $H_1(F;\Z)$ on which the Seifert form is given by a bilinear form that satisfies~\eqref{eq:Alex1} since any pair of such homology classes can be represented by once intersecting simple closed curve; see~\cite[Proposition~9]{FellerLewark_16} or~\cite[last paragraph of the proof of Proposition~6]{FellerMcCoy_15} for details.
Consequently, for the rest of the proof, we only concern ourselves with the Seifert form on $F$ and subgroups $H$ as described above.

The Seifert form of $H_1(F;\Z)$ with respect to the basis $([\alpha_1],\dots,[\alpha_{n-1}])$ is
\[
M_k=M_0+M_{\rm twist}=
\left(\begin{array}{ccccc}-1&-1&0&0&\\
0&-1&-1&0&\\
0&0&-1&-1&\\
&&& & \ddots\end{array}\right)
+k\left(\begin{array}{cccc}
4&4&4&\\
4&4&4&\cdots\\
4&4&4&\\
 & \vdots && \ddots
\end{array}\right);
\]
in particular, for $n=5$
\begin{equation}\label{eq:Mforp=5}M_k=\left(\begin{array}{cccc} 4k-1 & 4k-1 & 4k & 4k\\
4k & 4k-1 & 4k-1&4k\\
4k & 4k & 4k-1 & 4k-1\\
4k & 4k & 4k & 4k-1\end{array}\right).\end{equation}
We note that $M_0+M_0^T$ is negative definite. In fact, for $k=0$, $F$ is the minimal Seifert surface of the $T_{2,-n+1}$ torus link.

We have now reduced the problem to the following linear algebra question:
for $n\geq5$ and $k=1$, do there exist vectors $a$ and $b$ in $\Z^{n-1}$ such that
$a^TM_ka=0$, $a^TM_kb=0$, and $b^TM_ka=\pm1$? And, once we have such an $H$ for $n=5$, we have it for all $n\geq 5$ since $M_k$ for $n=5$ is the top-left $4\times4$ sub-matrix of $M_k$ for $n\geq 5$.
Hence, we conclude the proof by noting that the following pair of vectors has the desired property: $\left(a=( -1,  -1,   0,   1)^T, b=(4,   1,   2,  -4)^T\right)$.

We turn to the last assertion. Call $p = 2n-1$.
If $T_{2n-1,2n}$ bounds a locally-flat M\"obius band $M \subset B^4$, then the linking form of $\Sigma(T_{2n-1,2n})$ represents $\frac1p$ or $-\frac1p$ as a square, by Proposition~\ref{p:MY}.

By Lemma~\ref{l:surgerypresSigmatorus}, $\Sigma(2,2n-1,2n)$ bounds a $4$--manifold with $H_1=0$ and intersection form presented by $\big({\tiny\begin{array}{cc}n-1 & n \\ n & n-1\end{array}}\big)$, and therefore the linking form of $\Sigma(2,2n,2n+1)$ is presented by $\frac1p \big({\tiny\begin{array}{cc}n-1 & n \\ n & n-1\end{array}}\big)$. In particular, it represents $\frac{n-1}{p}$ as a square.

However, since $2(n-1) = 2n-2 \equiv -1 \pmod p$, the linking form represents $\frac{n-1}{p}$ if and only if it represents $-\frac{2}{p}$ as a square; since $p \equiv 5 \pmod 8$, by Lemma~\ref{l:presentingassquares}.\eqref{linking2mod4}, the linking form cannot represent $\frac1p$ nor $-\frac1p$ as a square.
\end{proof}

\subsection{Torus knots that do not bound M\"obius bands}\label{subsec:mob}

Recall that Batson~\cite{Batson} proved that $\gsmooth(T_{2n-1,2n}) = n-1$ for each $n \ge 2$; however, his result says nothing about $\gsmooth(T_{2n,2n+1})$. For this reason, for most of this section we focus on finding values of $n$ for which we can prove that $\gtop(T_{2n,2n+1}) > 1$.

%We generalize the result that $T_{4,5}\subset S^3$ does not bound a M\"obius band in $B^4$.

First we proof Proposition~\ref{p:T45} from the introduction; that is, we show that $T_{2n,2n+1}$ does not bound a M\"obius band if $2n+1$ is a prime congruent to $5$ modulo $8$.
%\begin{prop}\label{p:T45}
%Let $n\equiv 2 \pmod 4$ be a positive  integer such that $2n+1$ is a prime. Then $T_{2n,2n+1}$ does not bound a locally-flat M\"obius band in $B^4$.
%In particular, the knot $T_{4,5}$ does not bound a locally-flat M\"obius band in $B^4$.
%\end{prop}
The proof is essentially identical to the proof of the last assertion in Proposition~\ref{prop:gammatop<gammasmooth}. Instead of repeating the proof, we only outline the differences.

\begin{proof}[Proof of Proposition~\ref{p:T45}]
Let $p = 2n+1$. $\Sigma(T_{2n,2n+1})$ now bounds a $4$--manifold with intersection form presented by $\big({\tiny\begin{array}{cc}-n-1 & n \\ n & -n-1\end{array}}\big)$, and therefore the linking form represents $\frac{n+1}{p}$ as a square. Now the inverse of $n+1$ modulo $p$ is $2$ instead of $-2$, but since $p\equiv 5 \pmod 8$ the sign change has no impact.
\end{proof}

The next proposition implies Theorem~\ref{thm:nomob} when $n$ is a prime.

\begin{prop}\label{prop:T2p2kppm1doesnotboundMB}
For each odd prime $p$ there are infinitely many positive integers $k$ such that the knot $T_{2p,2kp \pm 1}$ does not bound a locally-flat M\"obius band in $B^4$.
\end{prop}

The statement means that for each choice of a sign there are infinitely many values of $k$ such that the statement is true; i.e. we do not claim that there are values of $k$ such that the statements holds with both signs. We prefer to leave the ambiguity in order to keep the notation lighter.

\begin{proof}
Let $q$ be a prime number with $q\equiv 1 \pmod 4$ and such that $p$ is not a square residue modulo $q$. We claim that we can always construct such a number.
Indeed, by quadratic reciprocity, $\jacobi{p}{q} = \jacobi{q}{p}$; so it suffices to choose $q$ such that $\jacobi{q}{p} = -1$. There are infinitely many such primes: it suffices to pick an integer $r$ such that $\jacobi{r}{p} = -1$ and look at the arithmetic progression $r+sp$, which contains infinitely many primes by Dirichlet's theorem.
Since $q\equiv 1 \pmod 4$, $\jacobi{-1}q = 1$, so that $\jacobi{-p}{q} = -1$, too.
In particular, for any positive integer $r$, neither $-p$ nor $p$ is a square modulo $qr$.

Let $h_0$ be any positive integer such that $2h_0p \pm 1 \equiv q \pmod{q^2}$. Let us look at the arithmetic progression $2h_0p \pm 1 + hpq^2$, with $h > 0$. Since $\gcd(2h_0p\pm1, pq^2) = q$, we can re-write
\[
2h_0p \pm 1 + hpq^2 = q(a + hpq),
\]
where $\gcd(a,pq) = 1$; in particular, by Dirichlet's theorem there are infinitely many primes in the arithmetic progression $a+hpq$. Choose $h$ such that $r = a+hpq$ is a prime, and let $k = h_0 + q^2h$.
In particular, we have $2kp\pm 1 = qr$.

We claim that $T_{2p,2kp\pm 1}$ does not bound a locally-flat M\"obius band, and more precisely that $T_{2p,2kp\pm 1}$ violates the Murakami--Yasuhara criterion.

Since $qr = 2kp\pm 1$, $qr = \det T_{2p,2kp\pm 1}$; since $q$ and $r$ are distinct primes, $H_1(\Sigma(2,2p,qr)) \cong \Z/qr\Z$.
By tweaking the proof of Lemma~\ref{l:surgerypresSigmatorus}, we see that $\Sigma(2,2p,qr)$ has a surgery presentation for which the linking matrix is given by the following tridiagonal $2k\times 2k$ matrix:
\[
Q = \left({
\tiny{
\begin{array}{cccccccccccccccccccc}
-2 & 1  \\
1 & -2 \\
& & \ddots  \\
& & &  -2 & 1 & 0 & 0\\
& & & 1 & \pm p - 1 & \pm p & 0\\  
& & & 0 & \pm p & \pm p - 1 & 1\\
& & & 0 & 0 & 1 &- 2\\
& & & & & & & \ddots \\
& & & & & & & & -2 & 1 \\
& & & & & & & & 1 & -2 \\
\end{array}}
}
\right).
\]
Since $H_1(\Sigma(2,2p,qr))$ is cyclic, it suffices to compute one non-trivial square in the linking form $\lambda$; by an explicit inductive computation, the first entry of the matrix $-Q^{-1}$, which is the matrix that represents the linking form, is $\frac{qr\mp p}{qr}$.

Since $\jacobi{p}{q} =\jacobi{-p}{q}= -1$ by choice, and since $\lambda$ represents $\mp\frac{p}{qr}$ as a square by the previous computation, $\lambda$ does not represent $\frac{1}{qr}$ nor $-\frac{1}{qr}$ as a square. Thus, by Proposition~\ref{p:MY}, $T_{2p,2kp\pm1}$ is not the boundary of a locally-flat M\"obius band.
\end{proof}

We want to highlight the limitations of the proposition above;
first of all, when $\det K$ is not square-free, Proposition~\ref{p:MY} above does not apply. The original criterion by Murakami and Yasuhara~\cite[Corollary~2.7]{MurakamiYasuhara} does still apply, but it yields a weaker obstruction. (The slogan is ``the proposition is true up to metabolisers''.)

Secondly, when $\det K$ is not a prime, it becomes (slightly) harder to determine whether $\pm 1/{\det K}$ is represented as a square.
Thirdly, there are shortcomings to applying the result even when $|{\det K}| =: q$ is a prime: if $-1$ is not a square residue modulo $q$ (equivalently, if $q \equiv 3 \pmod 4$), then for algebraic reasons either $1/q$ or $-1/q$ is always represented by a square. So, for instance, we cannot directly conclude anything about the existence of a M\"obius band in $B^4$ whose boundary is $T_{6,7}$. However, we can find an alternative to Proposition~\ref{p:T45}.

\begin{prop}\label{p:T67}
Let $n \equiv 3 \pmod 4$ be an integer such that $2n+1$ is a prime and ${n+1}$ is not a square.
Then $T_{2n,2n+1}$ does not bound a \emph{smooth} M\"obius band in $B^4$.
In particular, $T_{22,23}$ does not bound a smooth M\"obius band in $B^4$.
\end{prop}

Note that there are infinitely many integers satisfying the three conditions in the statement, by Dirichlet's density theorem on arithmetic progessions of primes.

\begin{proof}
We know from Lemma~\ref{l:surgerypresSigmatorus} that $Y \coloneqq \Sigma(2,2n,2n+1) = \Sigma(T_{2n,2n+1})$ bounds a spin negative definite $4$--manifold $W$ with second Betti number $2$.
By successively blowing up $W$, we obtain the canonical negative plumbing $P$ whose boundary is $Y$, according to Neumann~\cite{Neumann}; call $\Gamma$ the associated weighted graph (which is a three-legged star-shaped graph, in this case). Ozsv\'ath and Szab\'o computed correction terms of $Y$ starting from the plumbing graph $\Gamma$~\cite{OSz-plumbing} as follows.

Let $L$ be the intersection lattice of $P$, and fix a coset in ${\rm Char}(L)/2L$ (recall that the set ${\rm Char}(L)$ of characteristic covectors of $L$ is a $2L$--torsor). Since cosets in ${\rm Char}(L)/2L$ are in bijection with spin$^c$ structures on $Y$, we will denote the coset by the spin$^c$ structure $\ft$ it corresponds to. Then:
\begin{equation}\label{e:OSz-plumbing}
%d(Y,\ft) = \max_{\xi \in \ft} \frac{\xi^2 + \rank L}4.
d(Y,\ft) = d(L,\ft) \coloneqq \max_{\xi \in \ft} \frac{\xi^2 + \rank L}4.
\end{equation}

We make an easy observation here: if $L = \langle -1 \rangle \oplus L'$, then the inclusion $L'\to L$ induces a bijection $j: {\rm Char}(L)/2L \to {\rm Char}(L')/2L'$, and it is easy to verify that
$d(L,\ft) = d(L',j(\ft))$.
%\[
%\max_{\xi \in \ft} \frac{\xi^2 + \rank L}4 = \max_{\xi \in j(\ft)} \frac{\xi^2 + \rank L'}4.
%\]
This implies that, since $P$ is a blow-up of $W$ and the intersection from changes by taking the direct sum with $\langle -1 \rangle$ under blow-ups, we can do the maximisation on the intersection lattice of $W$ (which has rank $2$), rather than on the intersection lattice of $P$.

To unravel~\eqref{e:OSz-plumbing}, let $Q$ be the $2\times 2$ matrix $\big({\tiny\begin{array}{cc}- n - 1& n\\n& -n - 1\end{array}}\big)$. Since the entries on the diagonal are both even, characteristic covectors are of the form $2Q^{-1}\eta^T$, where $\eta = (\eta_1,\eta_2)$ is an integer vector. The maximisation then reads:
\begin{equation}\label{e:explicitd}
d(Y,\ft) = \max_{\xi \in \ft} \frac{\xi^2 + \rank L}4 = \max_{2Q^{-1}\eta^T \in \ft} {\eta}\,Q^{-1}\eta^T + \frac12 = \frac12 - (\eta_1 + \eta_2)^2 - \frac{\eta_1^2 + \eta_2^2}{2n+1}.
\end{equation}
Note that the quantity on the right-hand side is \emph{negative} as soon as $\eta_1+\eta_2 \neq 0$.

Suppose that $T_{2n,2n+1}$ bounds a (locally-flat) M\"obius band $M$ in $B^4$. Then $Y$ bounds a $4$--manifold $Z$ with $b_2(Z) = 1$, namely  the double cover of $B^4$ branched over $M$. If $M$ is smoothly embedded, then $Z$ is a \emph{smooth} $4$--manifold.

Since $2n+1$ is a prime (and in particular square-free), the intersection form of $Z$ is $\langle\pm(2n+1)\rangle$
If the intersection form of $Z$ is represented by the $1\times 1$ matrix $Q_Z = (+2n+1)$, the linking form is presented by the matrix $-Q_Z^{-1} = (-\frac1{2n+1})$, so that the linking form of $Y$ is $\langle -\frac1{2n+1}\rangle$, and therefore it always represents $-\frac1{2n+1}$ as a square.

Since $2n+1 \equiv 7 \pmod 8$, from Lemma~\ref{l:presentingassquares}.\eqref{linking3mod4},  $Z$ cannot be positive definite, hence the intersection form of $Z$ is $\langle-2n-1\rangle$.
However, Ozsv\'ath and Szab\'o~\cite[Theorem~9.6]{OSz-absolutely} proved, under these assumptions, for each spin$^c$ structure $\fs$ on $Z$ which restricts to $\ft$ on $Y$, that
\begin{equation}\label{e:OSz-inequality}
\frac{c_1(\fs)^2 + 1}4 \le d(Y,\ft),
\end{equation}
and that the two sides are congruent modulo $2$.

Let us focus on the case where $\langle c_1(\fs), H_2(Z) \rangle = \Z$ (this is possible since the intersection form of $Z$ is odd, and therefore there is such a spin$^c$ structure; in fact there are exactly two, which are conjugate). Then $c_1(\fs)^2 = -\frac{1}{2n+1}$, and therefore
%\[
%\frac{c_1(\fs)^2 + 1}{4}  = \frac{n}{4n+2} > 0.
%\]
$\frac{c_1(\fs)^2 + 1}{4}  = \frac{n}{4n+2} > 0$.

It follows from~\eqref{e:OSz-inequality} that $d(Y,\ft) > 0$, and therefore, from~\eqref{e:explicitd}, that $\ft$ corresponds to $Q^{-1}\eta^T$ with $\eta_1 + \eta_2 = 0$. In particular,
%\[
%d(Y, \ft) = \frac12 - \frac{2x^2}{2n+1}
%\]
$d(Y, \ft) = \frac12 - \frac{2x^2}{2n+1}$
for the integer $x=\eta_1$.

We now use the congruence condition in~\eqref{e:OSz-inequality}. We have (the reduction modulo $\frac12$ of) the congruence condition (modulo $2$) telling us that
$-1 \equiv -8x^2 \pmod{2n+1}$.
However, if $\frac{n+1}4$ is not a square, then the smallest positive integer solution $x$ of this congruence has $x > \sqrt{\frac{n+1}4}$, and therefore
\[
d(Y,\ft) = \frac12 - \frac{2x^2}{2n+1} < \frac12 - \frac{n+1}{4n+2} = \frac{n}{4n+2} = \frac{c_1(\fs)^2 + 1}{4},
\]
which contradicts~\eqref{e:OSz-inequality}.
\end{proof}

Recall that $2$--bridge links are links $L \subset \R^3 \subset S^3$ such that the restriction of the $z$--function is Morse with two minima and two maxima. The double cover of $S^3$ branched over a two $2$--bridge link is a lens space, and two $2$--bridge links are isotopic if and only if their branched covers are homeomorphic. We refer to $K_{p/q}$ as the unique $2$--bridge link whose double cover is the lens space $L(p,q)$; note that $K_{p/q}$ is a knot if and only if $p$ is odd, and that $p = |{\det K_{p/q}}|$.

\begin{prop}\label{p:2bridge}
For each prime $p\equiv 7 \pmod 8$, $p > 7$, the $2$--bridge knot $K_{p/(p-2)}$ does not bound a \emph{smooth} M\"obius band in $B^4$. The knot $K_{15/13}$ does not bound a \emph{locally-flat} M\"obius band.
\end{prop}

\begin{proof}
Suppose that $K_{p/(p-2)}$ bounds a smoothly embedded M\"obius band $M$ in $B^4$; then the double cover of $B^4$ branched over $M$ is a smooth $4$--manifold $Z$ with $b_2(Z) = 1$ whose boundary is a lens space, namely $\Sigma(K_{p/(p-2)}) = L(p,p-2)$. Since $p$ is square-free, the intersection form of $Z$ is $\langle \pm p \rangle$.

Recall that the linking form of $L(p,p-2)$ is $\langle \frac{2-p}p \rangle = \langle \frac{2}p \rangle$. Since $p\equiv 7 \pmod 8$, we know from Lemma~\ref{l:presentingassquares}.\eqref{linking3mod4} that the linking form of $L(p,p-2)$ must present $-\frac1p$, but cannot present $\frac1p$.
It follows, as in the proof of~\ref{p:T67} above, that $Z$ is positive definite, i.e. that its intersection form is $\langle +p \rangle$.

Gluing $-Z$ and the negative definite plumbing $P$ whose boundary is $L(p,p-2)$, we obtain a smooth, negative definite $4$--manifold $X$. In particular, the intersection form embeds with co-rank $1$ in a diagonal lattice, by Donaldson's diagonalization theorem~\cite{Donaldson}.

Recall that the negative definite plumbing of $L(p,p-2)$ is determined by the negative continued fraction expansion of $p/(p-2) = [2,\dots,2,3]$, where the string of $2$s has length $N-2 = (p-3)/2$. However, if $p > 7$ the string of $2$s has a unique embedding, namely---in some basis $e_1,\dots,e_N$ of $\Z^N$---$e_1-e_2,\dots,e_{N-2} - e_{N-1}$.
Since $N \ge 2$ by assumption, there is no vector in $\Z^N$ of self-intersection $-3$ that intersects the chain (algebraically) once in the last vector, which contradicts our assumption.

To prove the assertion about locally-flat M\"obius bands bounding $K_{15/13}$, we observe that the previous argument gives an embedding of the intersection form of $P$ into a negative definite lattice of rank $8$. There are only two such lattices, namely $\Z^8$ and $E_8$. We proved above that $P$ does not embedding into $\Z^n$; since $P$ contains a class of square $-3$, it cannot embed into the even lattice $E_8$ either. Therefore, $K_{15/13}$ does not bound a locally-flat M\"obius band.
\end{proof}
